Efficient Training of Convolutional Neural Nets on Large Distributed Systems

Deep Neural Networks (DNNs) have achieved im- pressive accuracy in many application domains including im- age classification. Training of DNNs is an extremely compute- intensive process and is solved using variants of the stochastic gradient descent (SGD) algorithm. A lot of recent research has focussed on improving the performance of DNN training. In this paper, we present optimization techniques to improve the performance of the data parallel synchronous SGD algorithm using the Torch framework: (i) we maintain data in-memory to avoid file I/O overheads, (ii) we present a multi-color based MPI Allreduce algorithm to minimize communication overheads, and (iii) we propose optimizations to the Torch data parallel table framework that handles multi-threading. We evaluate the performance of our optimizations on a Power 8 Minsky cluster with 32 nodes and 128 NVidia Pascal P100 GPUs. With our optimizations, we are able to train 90 epochs of the ResNet-50 model on the Imagenet-1k dataset using 256 GPUs in just 48 minutes. This significantly improves on the previously best known performance of training 90 epochs of the ResNet-50 model on the same dataset using 256 GPUs in 65 minutes. To the best of our knowledge, this is the best known training performance demonstrated for the Imagenet- 1k dataset.

==> sgd.tex <==
%
% SGD algorithm
% Data parallel distributed SGD
% Typical networks (deep and very deep neural networks)
% Async SGD (DownPour). Communication overheads in VGG
% Table of parameter sizes and batch computation times
% High throughput allreduce a solution to very deep networks 
% parallel I/O to load data into memory
%

In the stochastic gradient descent approach, a leaner executes SGD on a
mini-batch of images to compute gradients ($\Delta W$), that are used
to update the parameter weights as shown in the equation below.  Here
$\gamma$, $L$ and $w_d$ are the momentum, learning rate and the weight
decay hyper parameters, respectively.

\[ v_{t} = \gamma * v_{t-1} + L * \Delta W\]
\[ W = (1 - w_d) * W - v_t\]

%%% equation
We developed a distributed SGD optimizer that is data-parallel and
synchronous. In a distributed SGD with $N$ leaners, where each leaner
executes a mini-batch of size $m$, the effective batch size is $m*N$
that increases as we use more learners for increased parallelism. The
larger batch size enables a higher computation to communication ratio
as the global gradient sums must be exected less frequently. It has
been shown that large batch sizes are not effective in converging the
ImageNet classification problem~\cite{}. 

The different DNN models vary in the type of the layers, the number of
layers and the total number parameters. These impact the computation
time per mini-batch and the total volume of communication to sum
gradients. Parameter servers~\cite{} have been studied in literature
to sum gradient contributions from the $N$ leaners. The time to sum
gradients in a paramter server given by the equation below.  Here B is
the link throughput of the network link connected to the paramter
server.

\[parameter~server~commmunication~time = \Delta W * N / B\]

Table~\ref{tab:dnn_weights} shows the size of the parameters and the
mini-batch computation time on 4x NVIDIA Pascal P100 GPUs. The table
also compares the time to execute gradient summing via the multi-color
MPI\_Allreduce call and the lower bound on the communication time with
a single parameter server connected to the network with 2x 100Gbps
bi-directional links.

\begin{table*}
\begin{center}
\begin{tabular}{c|c|c|c|c}
%\toprule
DNN Model  & Parameter Size & 4xP100 Batch time & Allreduce & Parameter Server\\ \hline
%\toprule
NiN~\cite{}        & 38.5MB  & 135 ms & 8.5  ms  & 49.3 ms \\ \hline
GoogleNet~\cite{}  & 75.3 MB & 269 ms & 12.7 ms  & 96   ms \\ \hline
VGG-16~\cite{}     & 550 MB  & 520 ms & 91   ms  & 700  ms  \\ \hline
%\bottomrule
\vspace{0.2cm}
\end{tabular}
\caption{A comparison of parameter sizes, min-batch 256 execution time in milliseconds and communication overheads on 16x POWER8 nodes with 64 GPUs}
\label{tab:dnn_weights}
\end{center}
\end{table*}

Note, from the Table~\ref{tab:dnn_weights}, relatively high
communication overheads with a paramter server vs multi-color
allreduce. We expect the parameter server technique to be a bottleneck
on a very deep neural networks such as VGG-16. Our approach takes
advantage of the per-to-peer collective communication library calls in
MPI to sum gradients across the POWER8 SMP nodes. Note even with the
very deep VGG-16 network the communication overhead in the multi-color
allreduce is more than 5x less than the batch execution time.

Within the SMP node the mini-batches are executed using the
cudnn.torch package. The torch DataParallelTable component is used to
schedule cudnn compute kernels on the multiple GPUs within each SMP
node. At the end of each mini-batch the NVIDIA NCCL library is used to
sum the gradients and contribute the result to the MPI\_Allreduce
call.



